Accelerating Monte Carlo Bayesian Inference via Approximating Predictive Uncertainty over Simplex

Estimating the predictive uncertainty of a Bayesian learning model is critical in various decision-making problems, e.g., reinforcement learning, detecting adversarial attack, self-driving car. As the model posterior is almost always intractable, most efforts were made on finding an accurate approximation the true posterior. Even though a decent estimation of the model posterior is obtained, another approximation is required to compute the predictive distribution over the desired output. A common accurate solution is to use Monte Carlo (MC) integration. However, it needs to maintain a large number of samples, evaluate the model repeatedly and average multiple model outputs. In many real-world cases, this is computationally prohibitive. In this work, assuming that the exact posterior or a decent approximation is obtained, we propose a generic framework to approximate the output probability distribution induced by model posterior with a parameterized model and in an amortized fashion. The aim is to approximate the true uncertainty of a specific Bayesian model, meanwhile alleviating the heavy workload of MC integration at testing time. The proposed method is universally applicable to Bayesian classification models that allow for posterior sampling. Theoretically, we show that the idea of amortization incurs no additional costs on approximation performance. Empirical results validate the strong practical performance of our approach.

==> app.tex <==
\section{Training Details}    

The network architecture of the meta-network and witness function network are shown in Figure \ref{fig:meta}.
Specifically, we assume the meta-network and the witness function are two MLPs and assume $w = \{\mathbf{W}_i\}_{i=1}^C$ and $v = \{\mathbf{V}_i\}_{i=1}^R$.
    %
    The first $R-C$ layers of $\Omega$ generates an intermediate feature vector $\mathbf{f}$ for an input $\xst$, i.e., $\mathbf{f}=\sigma(\mathbf{V}_{R-C}\sigma(\mathbf{V}_{R-C-1} \cdots \sigma(\mathbf{V}_1\xst)\cdots))$, where $\sigma(\cdot)$ is the non-linearity.
    %
    The $i$-th layer weights of witness function are then generated by $\mathbf{w}_i=\mathbf{V}_i\mathbf{f}$.
    %
    $\mathbf{w}_i$ is then transformed to $\mathbf{W}_i$ to fit the structure of witness function.
    
   \begin{figure}[H]
        \centering
        \includegraphics[width=\textwidth]{flowchart.pdf} % second figure itself
        \caption{A flowchart for training.}
    	\label{fig:meta}
    \end{figure}
    
%The complete training algorithm is presented in Algorithm \ref{algo:train}.
%    
%	\begin{figure}[h!]
%	\begin{algorithm}[H]
%		\caption{The algorithm to train OPU model.}
%		\label{algo:train}
%		\input{algo}
%    \end{algorithm}
%    \end{figure}

\section{Approximation Details}
	\label{approx}
	%
	In this section, we illustrate the details for using OPU to approximate Bayesian logistic regression,
	% 
	Bayesian neural networks and Gaussian process classification.
	%
	Under some contexts, we use $\mb{X}$ and $\mb{Y}$ to collectively denote the inputs and outputs respectively for previous $\D$.
	
	\subsection{Bayesian Logistic Regression}
	
	The Polya-Gamma (PG) scheme~\citep{polson2013bayesian} is a data augmentation strategy that allows for a closed-form Gibbs sampler.
	%
	In binary classification, i.e., $y_n \in \mathcal{Y} = \{1, 0\}$, 
	% 
	let $\bg{\theta}$ be the regression coefficients with a Gaussian conditional conjugate prior
	%
	$p(\bg{\theta})\sim\mathcal{N}(\mb{0},\bg{\Lambda}^{-1})$.
	%
	The PG-augmented Gibbs sampler is composed of the following two conditionals,
	%
	\begin{eqnarray}
	\omega_n|\bg{\theta}, \mb{x}_n & \sim & \text{PG}(1, \mb{x}_n^{\mathsf{T}}\bg{\theta}) \\
	\bg{\theta}|\bg{\omega}, \D    & \sim & \mathcal{N}(\mb{m}_{\omega},\mb{V}_{\omega}),
	\end{eqnarray}
	%
	where $\omega_n$ is the augmenting data corresponding to the $n$th data point. The posterior conditional variance and mean are given by
	%
	$\mb{V}_\omega = (\mb{X}^\mathsf{T}\Omega\mb{X} + \bg{\Lambda}^{-1})^{-1}$ and
	%
	$\mb{m}_\omega=\mb{V}^{-1}_{\omega}(\mb{X}^\mathsf{T}(\mb{y}-\frac{1}{2}))$, respectively.
	%
	
	Given this results we will be able to collect samples from the posterior after a burn-in period.
	%
	The posterior samples $\{\bg{\theta}\}_{s=1}^S$, together with dataset $\D^\prime$,
	%
	are used to train our approximation with OPU goal defined in the main article.
	%
	
	As an MCMC method, the PG augmentation scheme offers accurate samples.
	%
	Other alternative methods such as local variational approximation can be employed,
	%
	which are much faster but sacrifice accuracy.
	
	%
	\subsection{Monte Carlo Dropout}\label{MCDP}
	
	A neural network with dropout applied before every weight layer was shown to be an approximation to 
	%
	probabilistic deep Gaussian process (GP)~\citep{gal2016dropout}.
	%
	Let $q(\bg{\theta})$ to be the approximate distribution to the GP posterior.
	%
	Here, $\bg{\theta}=\{\mb{\Theta}_i\}_{i=1}^L$ and $\mb{\Theta}_i$ is a parameter matrix of dimensions $K_i\times K_{i=1}$ for NN layer $i$.
	%
	In this approximation, $q(\bg{\theta})$ can be defined through direct modification:
	%
	\begin{align}
	\bg{\Theta}_i = \mb{M}_i \diag([z_{i,j}]_{i=1}^{K_i}),
	\end{align}
	% 
	where $z_{i,j}\sim \bern(p_i)$ for $i\in[L]$ and $j \in [K_{i-1}]$, given some prior dropout probabilities $p_i$ and
	% 
	matrices $\bg{\Theta}_i$ are treated as variational parameters.
	%
	The binary variable $z_{i,j} = 0$ indicates that unit $j$ in layer $i-1$ being dropped out as an input to layer $i$.
	%
	The predictive mean of this approximation is given by
	% 
	$\mathbb{E}[\yst | \xst] \approx \frac{1}{S}\sum_{s=1}^S f(\xst,\hat{z}_{1,s},\dots,\hat{z}_{L,s})$, which hence referred to as MC dropout (MCDP).
	%
	
	We use OPU to approximate the uncertainty induced by $q(\bg{\theta})$.
	%
	A sample in the MC ensemble
	is given by $\bg{\theta}_s=\{\bg{\Theta}_{i,s}\}_{i=1}^L=\mb{M}_i \diag([z_{i,j}]_{i=1}^{K_i})$.
	%
	%To get the MAP estimation of $\bg{\theta}$ is not realistic (optimal $p_i=1$~\cite{gal2016uncertainty}).
	%
	We set $\bg{\phi}_1=\{\bg{\Phi}_i\}_{i=1}^LZ$
	%=\{\bg{\Phi}_i\}_{i=1}^L$
	to the mean of $\bg{\theta}_s$, i.e.,
	% 
	$\bg{\Phi}_i=\frac{1}{S}\sum_{s=1}^S\bg{\Theta}_{i,s}=\mb{M}_i \frac{1}{S} \sum_{s=1}^S \diag([z_{i,j,s}]_{i=1}^{K_i})$.
	%
	
	MCDP provides a simple way of approximating Bayesian inference through dropout sampling.
	%
	However, it still introduces a variational approximation to exact Bayesian posterior.
	%
	Therefore, we further include a more accurate way to generate MC ensemble - stochastic gradient Langevin dynamics (SGLD).
	% 
	
	\subsection{Vanilla SGLD}
	
	SGLD enables mini-batch MC sampling from the posterior via adding a noise step to SGD~\citep{welling2011bayesian}.
	%
	We choose the ``vanilla'' version of SGLD in our approximation.
	%
	Specifically, we start training of $f_{\bthe}(\cdot)$ from $\bthe^{(0)}$.
	%
	In each epoch with mini-batch size $B$, 
	% 
	\begin{align}\label{eq:sgld}
	\bthe^{(t+1)} & = \bthe^{(t)} + \epsilon_t \nabla \log p(\bthe^{(t)} | \D) + \eta_t \\
	& = \bthe^{(t)} + \epsilon_t \nabla( \log p(\bthe^{(t)}) + \sum_{b=1}^B \log p(\mb{y}_b | \mb{x}_b, \bthe^{(t)})) + \eta_t,
	\end{align}
	%
	where $B$ is the size of a mini-batch and $\eta_t\sim\mathcal{N}(0,2\epsilon_t\mb{I})$.
	%
	After SGLD converges at step $T$, the samples $\bthe_s = \bthe^{(T+s)}$ is collected by
	% 
	running the training process for another $S$ iterations.
	%
	We use averaged samples as parameter of $h$, i.e., $\phi_1=\frac{1}{S}\sum_{s=1}^S\bg{\theta}_s$ and
	% 
	train OPU by Eq.~\ref{eq:opt} with this ensemble.
	
% 	\begin{algorithm}[tbh]
% 		\caption{\sc{OPU Distilled SGLD}}
% 		\label{alg:online}
% 		\begin{algorithmic}
% 			\STATE {\bfseries Input:}  $\D = \{(\mb{x}_n, \mb{y}_n)\}_{n=1}^N$, number of iteration $T$, learning schedule of teacher $\epsilon_t$ and student $\rho_t$, cache for samples $C=\{\bg{\theta}_s\}_{s=1}^S$
% 			\REPEAT
% 			\STATE // \, training teacher (SGLD step) \, //
% 			\STATE Sample one data point $\xst$
% 			\STATE Update $\bg{\theta}^{(t+1)}$ via Eq.~\ref{eq:sgld} and cache $C\leftarrow C\cup\bg{\theta}^{(t+1)}$
% 			\STATE $C\leftarrow C \setminus \{\bg{\theta}_1\}$ \textbf{if} $|C|>S$ 	
% 			\STATE // \, training student (OPU step) \, //
% 			\STATE $\bg{\phi}^{(t+1)} := \bg{\phi}^t - \rho_t(- S^{-1}\sum_{s}\nabla\ln q(f(\xst;\bg{\theta}_s)|\alpha(\xst; \bg{\phi})))$
% 			\UNTIL{$t=T$}
% 		\end{algorithmic}
% 	\end{algorithm}
% 	% 
	
% 	An interesting extension of this approximation is stochastically training SGLD together with OPU.
% 	%
% 	Although it is not the main purpose of this paper, we show steps of this extension, to elaborate the idea of OPU by a comparison with Bayesian dark knowledge (BDK)~\cite{balan2015bayesian}.
% 	%
% 	As shown in Algorithm~\ref{alg:online}, we maintain a cache of parameter samples as the MC ensemble to update OPU.
% 	%
% 	At each step, the cache is updated after the SGLD teacher is trained, then OPU is updated with the MC ensemble.
% 	%
% 	BDK also provides an online algorithm that ``distills'' SGLD.
% 	%
% 	The difference is that, when the BDK algorithm trains the student network,
% 	% 
% 	it uses only one parameter sample but much more data points than those for training the teacher within one iteration.
% 	%
% 	This shows the difference between OPU and BDK:
% 	% 
% 	OPU explicitly approximates the teacher's uncertainty on each $\xst$ by fitting a Dirichlet on a set of teacher's outputs over the simplex.
% 	%
% 	BDK may implicitly approximate the predictive uncertainty $p(\yst | \xst, \D)$ which comes from a mixture of data uncertainty and model uncertainty.
	
	
	\subsection{Monte Carlo Gaussian Process}
	\label{GP}
	
	We apply the OPU framework to the GP framework, which demonstrate its use on a non-parametric classifier.
	%
	Let data $\D$ be split into as input matrix $\mb{X}$ and output matrix $\mb{Y}$.
	%
	We consider GP prior over the space of functions, i.e.,
	%
	$\bg{\mu} \sim \mathcal{GP}(0, \mathcal{K})$.
	%
	where $\mathcal{K}$ is a positive definite kernel controlling the prior belief on smoothness.
	%
	Existing techniques allow us to compute $q(\bg{\mu})$ which approximates $p(\bg{\mu} | \D)$ and 
	% 
	is comparable to previous $q(\bthe)$ under a parametric model.
	% 
	In a classification task, the posterior $p(\bg{\mu}|\D)$ can be sampled via MCMC~\citep{hensman2015mcmc}
	% 
	or approximated, e.g., via variational approximation~\citep{hensman2015scalable}.
	%
	Let $\bg{\mu}^\ast$ be a shorthand for $\bg{\mu}_{\xst}$ and $\pist$ is then defined as $\mathcal{S}(\bg{\mu}^\ast)$.
	% 
	If Gaussian variational approximation is used, the marginal posterior $p(\bg{\mu}^\ast | \xst, \D)$ at $\xst$
	% 
	induces a logistic-normal distribution for $p(\pist | \xst, \D)$.
	%
	% The predictive distribution is then
	% % 
	% \begin{equation}
	% p(\pi^\ast | \xst, \D_1) = \int p(\pi^\ast | \xst, \bg{\mu})p(\bg{\mu}|\D) \,\mathrm{d}\bg{\mu}
	% \end{equation}
	%
	In our approximation, we obtain samples $\{\bg{\mu}^\ast_s\}_{s=1}^S$ from $p(\bg{\mu}^\ast| \xst, \D)$.
	%
	The optimization goal is the same as that in the NN case with a different target distribution defined as 
	%
	\begin{align}
	\hat{p}(\pist | \xst, \D) = \frac{1}{S}\sum_{s=1}^S \delta(\pist - \mathcal{S}(\bg{\mu}^\ast_s)).
	\end{align}

\section{More experiment details}

Based on our observation, the results of OPU on three metrics (AUROC, AUPR and acc) are deterministic so we do not introduce error bar.
%
We run the trial of running time for 5 times and show the results with error bar as in Section 4.
%

We also do some tests for training OPU with KL divergence. 
%
The training is always damaged by ``NaN'' output of the neural network, which stops the training process. (7 times out of 10 trials, on OPU-SGLD)
%
This might due to the instable gradient provided by KL divergence.
%
By contrast, with proper choice of meta-network structure and learning rate (Section 4), using Wasserstein metric does not suffer from this.
%

